Low Thrust Trajectory Design Using A Semi-Analytic Approach

Space missions that use low-thrust propulsion technology are becoming increasingly popular since they utilize propellant more efficiently and thus reduce mission costs. However, optimizing continuous-thrust trajectories is complex, time-consuming, and extremely sensitive to initial guesses. Hence, generating approximate trajectories that can be used as reliable initial guesses in trajectory generators is essential. This paper presents a semi-analytic approach for designing planar and three-dimensional trajectories using Hills equations. The spacecraft is assumed to be acted upon by a constant thrust acceleration magnitude. The proposed equations are employed in a Nonlinear Programming Problem (NLP) solver to obtain the thrust directions. Their applicability is tested for various design scenarios like orbit raising, orbit insertion, and rendezvous. The trajectory solutions are then validated as initial guesses in high-fidelity optimal control tools. The usefulness of this method lies in the preliminary stages of low-thrust mission design, where speed and reliability are key.

==> LongAbstract.tex <==
% use paper, or submit
% use 11 pt (preferred), 12 pt, or 10 pt only

% \documentclass[letterpaper, preprint, paper,11pt]{AAS}	% for preprint proceedings
%\documentclass[letterpaper, paper,11pt]{AAS}		% for final proceedings (20-page limit)
%\documentclass[letterpaper, paper,12pt]{AAS}		% for final proceedings (20-page limit)
%\documentclass[letterpaper, paper,10pt]{AAS}		% for final proceedings (20-page limit)
%\documentclass[letterpaper, submit]{AAS}			% to submit to JAS

\usepackage{bm}
\usepackage{amsmath}
\usepackage[utf8x]{inputenc}
\usepackage{multirow}
\usepackage{breqn}
\usepackage{subfigure}
\usepackage{placeins}
%\usepackage[notref,notcite]{showkeys}  % use this to temporarily show labels
\usepackage[colorlinks=true, pdfstartview=FitV, linkcolor=black, citecolor= black, urlcolor= black]{hyperref}
\usepackage{overcite}
\usepackage{footnpag}			      	% make footnote symbols restart on each page



\PaperNumber{XX-XXX}



\begin{document}

\title{Low Thrust Trajectory Design Using A Semi-Analytic Approach}

\author{Madhusudan Vijayakumar\thanks{Graduate Student, Department of Aerospace Engineering, Iowa State University, USA.},  
Ossama Abdelkhalik\thanks{Corresponding Author, Associate Professor, Department of Aerospace Engineering, Iowa State University, Ames, Iowa 50011, AIAA senior member.}
}

\maketitle{} 		

\begin{abstract}
Space missions that use low thrust propulsion technology are becoming increasingly popular since they utilize propellant more efficiently and thus reduce mission cost. However, the optimization of continuous-thrust trajectories is complex, time consuming and extremely sensitive to initial guesses. Hence, generating approximate trajectories that can be used as reliable initial guesses in trajectory generators is essential. This paper presents a semi-analytic approach for the design of both planar and three-dimensional trajectories using Hills equations for a constant thrust acceleration magnitude. The proposed equations are employed in a Nonlinear Programming Problem (NLP) solver to obtain the thrust directions. Their applicability is tested for various design scenarios like orbit raising, orbit insertion and rendezvous. The trajectory solutions are then validated as initial guesses in high fidelity optimal control tools. The usefulness of this method lies in preliminary stages of low-thrust mission designs where speed and reliability is key.
\end{abstract}

\section{Low Thrust Analytic Approximation of Hill's Equations}

The Clohessy-Wiltshire equations, also referred to as Hill's equations are a set of linear, time invariant differential equations used to describe the motion of a spacecraft relative to a reference orbit. The reference orbit is usually a circle and the corresponding coordinate frame of the relative motion is shown in Fig ~\ref{fig:CF}. The $X-Y-Z$ frame represents the inertial coordinate system and $x-y-z$ represents the Hill's frame. In our case, $X-Y-Z$ represents the Earth Centered Inertial Frame (ECI). The $x$, $y$ and $z$ coordinates of the Hill's frame are the radial, along-track and cross-track displacements of the spacecraft relative to the reference orbit.
\begin{figure}[h!]
  \centering
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/Relative_Frame.png}
    \caption{Coordinate Frames}
    \label{fig:CF}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/xyz.png}
    \caption{Hills Frame}
    \label{fig:Hills_Frame}
  \end{minipage}
\end{figure}
The primary goal is to obtain an analytic approximation. Consider the two-body Hill's equation as shown in Eq.~\eqref{CW_Eqn}.
\begin{subequations}
\label{CW_Eqn}
\begin{align}
     \ddot{x}-2\,x\,n^2 -2\,\dot{y} \,n &=a_x \label{eq:CW_x} \\
     \ddot{y} +2\,n\,\dot{x} &=a_y \label{eq:CW_y} \\
    \ddot{z} + z\,n^2 &= a_z \label{eq:CW_z}
    \end{align}
\end{subequations}
where, $a_x$, $a_y$ and $a_z$ are the components of the trust acceleration represented in the Hill's frame. Assume that the thrust acceleration has a constant magnitude and its components vary linearly such that the in-plane components start at an initial phase angle $\alpha_0$ and the out-of-plane component starts at an initial phase angle $\beta_0$ as show in Fig ~\ref{fig:Hills_Frame}. Let $k_1$ and $k_2$ be the rates at which the in-plane and the out-of-plane thrust acceleration components rotate in the Hill's frame. Then the thrust acceleration components can be represented as:
\begin{equation}
\begin{aligned}
    a_x &= a  \sin(\beta_0 - k_2t)cos(\alpha_0 - k_1t) \\
    a_y &= a\sin(\beta_0 - k_2t)sin(\alpha_0 - k_1t) \\
    a_z &= a\cos(\beta_0 - k_2t)
\end{aligned}
\end{equation}
The primary task is to obtain an approximate analytic solution of the  Clohessy-Wiltshire equations for spacecrafts employing continuous low thrust. One way to solve the second-order homogeneous differential equations in Eq.~\eqref{CW_Eqn}, is to use Laplace transform. The out-of-plane motion in Eq.~\eqref{eq:CW_z} is uncoupled from the in-plane motion i.e. only the $z$ component appears and is the simplest among them to solve. This equation resembles the equation of an undamped harmonic oscillator with a forcing (or input) function on the right-hand side. Taking the Laplace transform of \label{CW_z} and rewriting the equation we get:
\begin{equation}
\label{Z_laplace}
    Z\left(s\right)=\frac{{\dot{z} }_0 +s\,z_0 +\frac{a\,{\left(s\,\mathrm{cos}\left(\beta_0 \right)+k_2 \,\mathrm{sin}\left(\beta_0 \right)\right)}}{{k_2 }^2 +s^2 }}{n^2 +s^2 }
\end{equation}
where, $s$ is a complex number, $z_0$ and ${\dot{z}}_0$ are the z-component of the velocity vector at $t = 0$. Taking the inverse Laplace transform of Eq.~\eqref{Z_laplace} we obtain:
\begin{dmath}
    \label{zt_eqn}
    z(t) = \frac{{k_2 }^2 \,{\dot{z} }_0 \,\mathrm{sin}\left(n\,t\right)-n^3 \,z_0 \,\mathrm{cos}\left(n\,t\right)-n^2 \,{\dot{z} }_0 \,\mathrm{sin}\left(n\,t\right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    +\frac{a\,n\,\mathrm{cos}\left(n\,t\right)\,\mathrm{cos}\left(\beta_0 \right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    +\frac{a\,k_2 \,\mathrm{sin}\left(n\,t\right)\,\mathrm{sin}\left(\beta_0 \right)+{k_2 }^2 \,n\,z_0 \,\mathrm{cos}\left(n\,t\right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    -\frac{a\,\mathrm{cos}\left(k_2 \,t\right)\,\mathrm{cos}\left(\beta_0 \right)+a\,\mathrm{sin}\left(k_2 \,t\right)\,\mathrm{sin}\left(\beta_0 \right)}{{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
\end{dmath}
Differentiating the above equation we get: 
\begin{dmath}
\label{zdott_eqn}
    \dot{z}(t) = \frac{a\,k_2 \,\mathrm{cos}\left(k_2 \,t\right)\,\mathrm{sin}\left(\beta_0 \right)-a\,k_2 \,\mathrm{sin}\left(k_2 \,t\right)\,\mathrm{cos}\left(\beta_0 \right)}{{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    -\frac{n^3 \,{\dot{z} }_0 \,\mathrm{cos}\left(n\,t\right)-n^4 \,z_0 \,\mathrm{sin}\left(n\,t\right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    -\frac{a\,n^2 \,\mathrm{sin}\left(n\,t\right)\,\mathrm{cos}\left(\beta_0 \right)+{k_2 }^2 \,n^2 \,z_0 \,\mathrm{sin}\left(n\,t\right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
    +\frac{{k_2 }^2 \,n\,{\dot{z} }_0 \,\mathrm{cos}\left(n\,t\right)-a\,k_2 \,n\,\mathrm{cos}\left(n\,t\right)\,\mathrm{sin}\left(\beta_0 \right)}{n\,{\left(k_2 +n\right)}\,{\left(k_2 -n\right)}}
\end{dmath}
From Eq.~\eqref{zt_eqn} and Eq.~\eqref{zdott_eqn} notice that the out-of-plane motion is only influenced by $z$ and $\dot{z}$. Thus, we can write, 
\begin{equation}
\begin{aligned}
\label{eq:y_function}
    z(t) = f_z (z_0,\dot{z}_0,\beta_0,k_2,t) \\
    \dot{z}(t) = f_{\dot{z}} (z_0,\dot{z}_0,\beta_0,k_2,t)
    \end{aligned}
\end{equation}
On the contrary, Eq.~\eqref{eq:CW_x} and ~\eqref{eq:CW_y} highlights that the planar motion of the spacecraft along $x$ and $y$ directions are coupled to each other. The closed form analytic solution for the in-plane position and velocity are obtained as follows. Start from Eq.~\eqref{eq:CW_x} and differentiate it to get:
\begin{equation}
    \dddot{x}=2\,n\,\ddot{y} + 3\,n^2 \,\dot{x} + a\,k_1 \,\mathrm{sin}\left(\alpha_0 -k_1 \,t\right)\,\mathrm{sin}\left(\beta_0 -k_2 \,t\right) - a\,k_2 \,\mathrm{cos}\left(\alpha_0 -k_1 \,t\right)\,\mathrm{cos}\left(\beta_0 -k_2 \,t\right)
\end{equation}
Now, substitute $\ddot{y} = -2\,n\,\dot{x} + a\,\mathrm{sin}\left(\alpha_0 -k_1 \,t\right)\,\mathrm{sin}\left(\beta_0 -k_2 \,t\right)$ in the $\dddot{x}$ to get:
\begin{equation}
    \dddot{x} = -n^2 \,\dot{x} - a\,k_2 \,\mathrm{cos}\left(\alpha_0 -k_1 \,t\right)\,\mathrm{cos}\left(\beta_0 -k_2 \,t\right) + a\,\mathrm{sin}\left(\alpha_0 -k_1 \,t\right)\,\mathrm{sin}\left(\beta_0 -k_2 \,t\right)\,{\left(k_1 +2\,n\right)}
\end{equation}
Take the Laplace transform of the $\ddot{x}$ to get,
\begin{equation}
X\left(s\right)=\frac{{\ddot{x} }_0 +s\,{\dot{x} }_0 -3\,n^2 \,x_0 +s^2 \,x_0 +2\,n\,{\left(2\,n\,x_0 -a\,\eta_3 \right)}-a\,k_1 \,\eta_3-a\,k_2 \,\eta_4}{n^2 \,s+s^3 }\\
\end{equation}
where, \hfill 
\begin{center}
\begin{math}
    \begin{array}{cc}
\eta_1 =\frac{\mathrm{sin}\left(\alpha_0 +\beta_0 \right)\,{\left(k_1 +k_2 \right)}+s\,\mathrm{cos}\left(\alpha_0 +\beta_0 \right)}{2\,{\left({{\left(k_1 +k_2 \right)}}^2 +s^2 \right)}} & \eta_2 =\frac{s\,\mathrm{cos}\left(\alpha_0 -\beta_0 \right)+\mathrm{sin}\left(\alpha_0 -\beta_0 \right)\,{\left(k_1 -k_2 \right)}}{2\,{\left(s^2 +{{\left(k_1 -k_2 \right)}}^2 \right)}}\\
\eta_3 = \eta_1 - \eta_2 & \eta_4 = \eta_1 + \eta_2 \\ 
    \end{array}
\end{math}
    \end{center}
Now, taking the inverse Laplace transform transform and substituting $\ddot{x}_0$ from Eq.~\eqref{eq:CW_x} we get an expression for $x(t)$. Further differentiating the $x(t)$ equation, we can arrive an expression for the velocity $\dot{x}(t)$. Notice that both $x(t)$ and $\dot{x}(t)$ are only a function of the planar components of the initial states as shown in Eq.~\eqref{eq:x_function}. Detailed expressions for the position and velocity $x(t)$ and $\dot{x}(t)$ is presented in the Appendix.
\begin{equation}
\begin{aligned}
\label{eq:x_function}
    x(t) = f_x (x_0,\dot{x}_0,\alpha_0,\beta_0,k_1,k_2,t) \\
    \dot{x}(t) = f_{\dot{x}} (x_0,\dot{x}_0,\alpha_0,\beta_0,k_1,k_2,t)
    \end{aligned}
\end{equation}
By substituting the expression for $\dot{x}(t)$ from Eq.~\eqref{eq:x_function} into the Hill's equation in Eq.~\eqref{eq:CW_y}, one can easily obtain expressions for $\dot{y}(t)$ and $y(t)$ by successive integration with respect to time. This would result in both $y(t)$ and $\dot{y}(t)$ expressed as functions of the planar components of the initial states as shown in Eq.~\eqref{eq:y_function}. Detailed expressions for the position and velocity $y(t)$ and $\dot{y}(t)$ is presented in the Appendix.
\begin{equation}
\begin{aligned}
\label{eq:y_function}
    y(t) = f_y (x_0,\dot{x}_0,\dot{y}_0,\alpha_0,\beta_0,k_1,k_2,t) \\
    \dot{y}(t) = f_{\dot{y}} (x_0,\dot{x}_0,\dot{y}_0,\alpha_0,\beta_0,k_1,k_2,t)
    \end{aligned}
\end{equation}
Since the closed form analytic solution of the spacecraft states is obtained by the linearization of Hill's equations, it is important to verify the validity of the solution. One way to estimate the accuracy preserved by this method, is to examine variations in the position and velocity components of the spacecraft motion wrt to its actual intended motion. This can be easily done by numerically propagating the states of the spacecraft using the two-body equation of motion and comparing that with the analytic approximation of spacecraft states. This experiment was conducted for a series of initial conditions and for a range of initial orbits from all the way from LEO to GEO. However, only one of the cases is demonstrated here since the trends in different parameters remained the same. The spacecraft was placed in an initial circular orbit at an altitude of $300\,km$ above the Earth and was propagated for a three orbital periods. It was assumed that the spacecraft was acted upon by a constant magnitude thrust acceleration of $9e-7\,km/s^2$. The initial thrust steering angles were kept at $\alpha_0 = 45 \deg$ and $\beta_0 = 60$. Figure~\ref{fig:Err_xy} and ~\ref{fig:Err_z} show the variations of in-plane and out-of-plane motion of the spacecraft compared to numerical propagation. 
\begin{figure}[h!]
  \centering
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/Err_in_plane.jpg}
    \caption{Error in Planar Direction}
    \label{fig:Err_xy}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/Err_out_of_plane.jpg}
    \caption{Error In Z-direction}
    \label{fig:Err_z}
  \end{minipage}
\end{figure}
Note that the errors in spacecraft states are represented in the canonical units. From the series of these experiments the following observations were made. 1. The error in the decoupled out-of-plane motion are very small compared to the error in the in-plane motion. This can be associated with the fact that the sources for error in the $z$-direction is half as that of the $x-y$ plane. 2. Irrespective of the initial orbit, the error in the analytical approximation is negligible for propagation times up to $20\%$ of the orbital period of the reference orbit. Additionally, we noticed that the error in spacecraft states was small up to a relative distance of $120\,km$ from the reference orbit. Beyond these limits, the errors associated with the analytical approximation increases exponentially because of the limitations due to linearization of Hill's equations.

\section{Sample Numerical Results: Coplanar Transfer From LEO (300 km) to GEO (35,785 km)}\label{SecResults} 
%h_event = 15000

A low-thrust trajectory design problem from an initial circular low Earth orbit (LEO) at an altitude $h_i = 300 \,$ km to a final circular Geostationary Orbit (GEO) of altitude $h_f = 35,785\,km$  is studied in this section. This is a typical orbit insertion problem where the spacecraft is acted upon by a fixed magnitude of thrust acceleration while the direction is variable. For this problem, the parameters of the spacecraft's propulsion system are defined as follows: specific impulse Isp = $3300\,s$, initial spacecraft mass = $95\,kg$, thrust-to-weight ratio = $1e-4$ and maximum thrust limit = $0.0920\,N$ and constant thrust acceleration of Ta = $9.81e-7\,m/s^2$.

The trajectory solution provided by the proposed semi-analytic method is shown in Figure~\ref{fig:LEO_GEO_Traj}. 
\begin{figure}[h!]
  \centering
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/LEO_GEO_traj.jpg}
    \caption{Plot of Trajectory}
    \label{fig:LEO_GEO_Traj}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/LEO_GEO_Ta_zoom.jpg}
    \caption{Plot of Ta Components}
    \label{fig:LEO_GEO_Ta_zoom}
  \end{minipage}
\end{figure}
The spacecraft takes $45.44\,days$ to transfer from LEO to GEO performing $N_{rev,e} = 338 \,$ revolutions around the Earth. In doing so, it consumes $10.52\,kg$ of propellant and achieves a $\Delta V = 3.85 \,km/s$. The corresponding thrust profile is an oscillating sinusoid in the $x$ and $y$ direction. A section of this thrust profile is displayed as a zoomed-in view in Fig~\ref{fig:LEO_GEO_Ta_zoom}. Figures~\ref{fig:LEO_GEO_r_err} and ~\ref{fig:LEO_GEO_v_err} illustrate the errors associated with the position and velocity of the analytically approximate trajectory compared to numerical propagation. Additionally, Table~\ref{tab:Performance_Characteristics} provides a detailed list of the obtained solution characteristics.
\begin{figure}[h!]
  \centering
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/LEO_GEO_r_err.jpg}
    \caption{Plot of Position Error}
    \label{fig:LEO_GEO_r_err}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{Figures/LEO_GEO_v_err.jpg}
    \caption{Plot of Velocity Error}
    \label{fig:LEO_GEO_v_err}
  \end{minipage}
\end{figure}

\begin{table}[h!]
	\fontsize{10}{10}\selectfont
    \caption{Performance Characteristics of the Semi-Analytic Solution}
   \label{tab:Performance_Characteristics}
        \centering 
   \begin{tabular}{c | c } % Column formatting, 
      \hline 
        Parameters & Value \\ 
            \hline
        No. of revolutions & 338 \\
        Time of Flight (days) & 45.44 \\ 
        $\Delta V$ (km/s) & 3.85 \\
        Propellant Consumption (kg) & 10.52 \\
      \hline
   \end{tabular}
\end{table}

\FloatBarrier
\section*{Acknowledgement}
This paper is based upon work supported by NASA, Grant Number 80NSSC19K1642

\newpage
\section{APPENDIX-A}

Analytic expression for the in-plane motion of the spacecraft.
\begin{dmath}
x(t) = \frac{2\,{k_1 }^2 \,\sigma_1 -2\,{k_2 }^2 \,\sigma_1 -a\,{k_1 }^2 \,\sigma_6+a\,{k_2 }^2 \,\sigma_6+2\,{k_1 }^2 \,n^2 \,x_0}{\sigma_{10}}+\frac{-2\,{k_2 }^2 \,n^2 \,x_0 +a\,{k_1 }^2 \,\sigma_7-a\,{k_2 }^2 \,\sigma_7}{\sigma_{10}}+\frac{-2\,a\,k_1 \,n\,\sigma_6+2\,a\,k_2 \,n\,\sigma_6+2\,a\,k_1 \,n\,\sigma_7+2\,a\,k_2 \,n\,\sigma_7}{\sigma_{10}}-\frac{a\,k_1 \,\sigma_4 \,\sigma_7-a\,k_1 \,\sigma_2 \,\sigma_9-a\,k_2 \,\sigma_4 \,\sigma_7+a\,k_2 \,\sigma_2 \,\sigma_9+2\,a\,n\,\sigma_4 \,\sigma_7-2\,a\,n\,\sigma_2 \,\sigma_9}{\sigma_{14}}-\frac{a\,k_1 \,\sigma_5 \,\sigma_6-a\,k_1 \,\sigma_3 \,\sigma_8+a\,k_2 \,\sigma_5 \,\sigma_6-a\,k_2 \,\sigma_3 \,\sigma_8+2\,a\,n\,\sigma_5 \,\sigma_6-2\,a\,n\,\sigma_3 \,\sigma_8}{\sigma_{14}}-\frac{2\,n^5 \,{\dot{x} }_0 \,\sigma_{12}-2\,{k_1 }^4 \,\sigma_{11}\,\sigma_1 -2\,{k_2 }^4 \,\sigma_{11}\,\sigma_1 -2\,n^4 \,\sigma_{11}\,\sigma_1}{\sigma_{13}} + \frac{-4\,{k_1 }^2 \,n^3 \,{\dot{x} }_0 \,\sigma_{12}-4\,{k_2 }^2 \,n^3 \,{\dot{x} }_0 \,\sigma_{12}-a\,{k_1 }^4 \,\sigma_{11}\,\sigma_7-a\,{k_2 }^4 \,\sigma_{11}\,\sigma_7}{\sigma_{13}}+\frac{-2\,a\,n^4 \,\sigma_{12}\,\sigma_9+4\,{k_1 }^2 \,{k_2 }^2 \,\sigma_{11}\,\sigma_1 +4\,{k_1 }^2 \,n^2 \,\sigma_{11}\,\sigma_1 +4\,{k_2 }^2 \,n^2 \,\sigma_{11}\,\sigma_1}{\sigma_{13}}+\frac{ +2\,{k_1 }^4 \,n\,{\dot{x} }_0 \,\sigma_{12}+2\,{k_2 }^4 \,n\,{\dot{x} }_0 \,\sigma_{12}+a\,{k_1 }^4 \,\sigma_6\,\sigma_{11}+a\,{k_2 }^4 \,\sigma_6\,\sigma_{11}}{\sigma_{13}}+\frac{+2\,a\,n^4 \,\sigma_8\,\sigma_{12}+a\,k_1 \,n^3 \,\sigma_8\,\sigma_{12}-2\,a\,k_1 \,n^3 \,\sigma_6\,\sigma_{11}-a\,{k_1 }^3 \,n\,\sigma_8\,\sigma_{12}}{\sigma_{13}}+\frac{+2\,a\,{k_1 }^3 \,n\,\sigma_6\,\sigma_{11}+a\,k_2 \,n^3 \,\sigma_8\,\sigma_{12}-2\,a\,k_2 \,n^3 \,\sigma_6\,\sigma_{11}-a\,{k_2 }^3 \,n\,\sigma_8\,\sigma_{12}}{\sigma_{13}}+\frac{+2\,a\,{k_2 }^3 \,n\,\sigma_6\,\sigma_{11}-4\,{k_1 }^2 \,{k_2 }^2 \,n\,{\dot{x} }_0 \,\sigma_{12}-2\,a\,{k_1 }^2 \,{k_2 }^2 \,\sigma_6\,\sigma_{11}+2\,a\,k_1 \,n^3 \,\sigma_{11}\,\sigma_7}{\sigma_{13}}+\frac{-a\,k_1 \,n^3 \,\sigma_{12}\,\sigma_9-2\,a\,{k_1 }^3 \,n\,\sigma_{11}\,\sigma_7+a\,{k_1 }^3 \,n\,\sigma_{12}\,\sigma_9-2\,a\,k_2 \,n^3 \,\sigma_{11}\,\sigma_7}{\sigma_{13}}+\frac{+a\,k_2 \,n^3 \,\sigma_{12}\,\sigma_9+2\,a\,{k_2 }^3 \,n\,\sigma_{11}\,\sigma_7-a\,{k_2 }^3 \,n\,\sigma_{12}\,\sigma_9-2\,a\,{k_1 }^2 \,n^2 \,\sigma_8\,\sigma_{12}}{\sigma_{13}}+\frac{-a\,{k_1 }^2 \,n^2 \,\sigma_6\,\sigma_{11}-2\,a\,{k_2 }^2 \,n^2 \,\sigma_8\,\sigma_{12}-a\,{k_2 }^2 \,n^2 \,\sigma_6\,\sigma_{11}+2\,a\,{k_1 }^2 \,{k_2 }^2 \,\sigma_{11}\,\sigma_7}{\sigma_{13}}+\frac{+a\,{k_1 }^2 \,n^2 \,\sigma_{11}\,\sigma_7+2\,a\,{k_1 }^2 \,n^2 \,\sigma_{12}\,\sigma_9+a\,{k_2 }^2 \,n^2 \,\sigma_{11}\,\sigma_7+2\,a\,{k_2 }^2 \,n^2 \,\sigma_{12}\,\sigma_9}{\sigma_{13}}+\frac{+4\,a\,k_1 \,k_2 \,n^2 \,\sigma_8\,\sigma_{12}-2\,a\,k_1 \,k_2 \,n^2 \,\sigma_6\,\sigma_{11}+a\,k_1 \,{k_2 }^2 \,n\,\sigma_8\,\sigma_{12}-2\,a\,k_1 \,{k_2 }^2 \,n\,\sigma_6\,\sigma_{11}}{\sigma_{13}}+\frac{+a\,{k_1 }^2 \,k_2 \,n\,\sigma_8\,\sigma_{12}-2\,a\,{k_1 }^2 \,k_2 \,n\,\sigma_6\,\sigma_{11}-2\,a\,k_1 \,k_2 \,n^2 \,\sigma_{11}\,\sigma_7+4\,a\,k_1 \,k_2 \,n^2 \,\sigma_{12}\,\sigma_9}{\sigma_{13}}+\frac{+2\,a\,k_1 \,{k_2 }^2 \,n\,\sigma_{11}\,\sigma_7-a\,k_1 \,{k_2 }^2 \,n\,\sigma_{12}\,\sigma_9-2\,a\,{k_1 }^2 \,k_2 \,n\,\sigma_{11}\,\sigma_7+a\,{k_1 }^2 \,k_2 \,n\,\sigma_{12}\,\sigma_9}{\sigma_{13}}\\
\end{dmath}
%------------------------------------------------------------------------------------------------------------------------------------------------
\begin{dmath}
\dot{x}(t) = \frac{a\,k_1 \,\sigma_5 \,\sigma_8\,{\left(k_1 +k_2 \right)}+a\,k_2 \,\sigma_5 \,\sigma_8\,{\left(k_1 +k_2 \right)}+2\,a\,n\,\sigma_5 \,\sigma_8\,{\left(k_1 +k_2 \right)}}{\sigma_{15}}+\frac{+a\,k_1 \,\sigma_3 \,\sigma_6\,{\left(k_1 +k_2 \right)}+a\,k_2 \,\sigma_3 \,\sigma_6\,{\left(k_1 +k_2 \right)}+2\,a\,n\,\sigma_3 \,\sigma_6\,{\left(k_1 +k_2 \right)}}{\sigma_{15}}+\frac{a\,k_1 \,\sigma_4 \,\sigma_9\,{\left(k_1 -k_2 \right)}-a\,k_2 \,\sigma_4 \,\sigma_9\,{\left(k_1 -k_2 \right)}+2\,a\,n\,\sigma_4 \,\sigma_9\,{\left(k_1 -k_2 \right)}}{\sigma_{14}}+\frac{+a\,k_1 \,\sigma_2 \,\sigma_7\,{\left(k_1 -k_2 \right)}-a\,k_2 \,\sigma_2 \,\sigma_7\,{\left(k_1 -k_2 \right)}+2\,a\,n\,\sigma_2 \,\sigma_7\,{\left(k_1 -k_2 \right)}}{\sigma_{14}}-\frac{2\,n^6 \,{\dot{x} }_0 \,\sigma_{11}+2\,n^5 \,\sigma_{12}\,\sigma_1 -4\,{k_1 }^2 \,n^4 \,{\dot{x} }_0 \,\sigma_{11}+2\,{k_1 }^4 \,n^2 \,{\dot{x} }_0 \,\sigma_{11}}{\sigma_{17}}+\frac{-4\,{k_2 }^2 \,n^4 \,{\dot{x} }_0 \,\sigma_{11}+2\,{k_2 }^4 \,n^2 \,{\dot{x} }_0 \,\sigma_{11}-2\,a\,n^5 \,\sigma_{11}\,\sigma_9-4\,{k_1 }^2 \,n^3 \,\sigma_{12}\,\sigma_1 }{\sigma_{15}}+\frac{-4\,{k_2 }^2 \,n^3 \,\sigma_{12}\,\sigma_1 +2\,a\,n^5 \,\sigma_8\,\sigma_{11}+2\,{k_1 }^4 \,n\,\sigma_{12}\,\sigma_1 +2\,{k_2 }^4 \,n\,\sigma_{12}\,\sigma_1 }{\sigma_{17}}+\frac{-a\,{k_1 }^2 \,n^3 \,\sigma_{12}\,\sigma_7+2\,a\,{k_1 }^3 \,n^2 \,\sigma_{12}\,\sigma_7-a\,{k_2 }^2 \,n^3 \,\sigma_{12}\,\sigma_7-2\,a\,{k_2 }^3 \,n^2 \,\sigma_{12}\,\sigma_7}{\sigma_{17}}+\frac{+a\,k_1 \,n^4 \,\sigma_8\,\sigma_{11}+a\,k_2 \,n^4 \,\sigma_8\,\sigma_{11}+2\,a\,k_1 \,n^4 \,\sigma_6\,\sigma_{12}-a\,{k_1 }^4 \,n\,\sigma_6\,\sigma_{12}}{\sigma_{17}}+\frac{+2\,a\,k_2 \,n^4 \,\sigma_6\,\sigma_{12}-a\,{k_2 }^4 \,n\,\sigma_6\,\sigma_{12}-a\,k_1 \,n^4 \,\sigma_{11}\,\sigma_9+a\,k_2 \,n^4 \,\sigma_{11}\,\sigma_9}{\sigma_{17}}+\frac{-2\,a\,{k_1 }^2 \,n^3 \,\sigma_8\,\sigma_{11}-a\,{k_1 }^3 \,n^2 \,\sigma_8\,\sigma_{11}-2\,a\,{k_2 }^2 \,n^3 \,\sigma_8\,\sigma_{11}-a\,{k_2 }^3 \,n^2 \,\sigma_8\,\sigma_{11}}{\sigma_{17}}+\frac{-2\,a\,k_1 \,n^4 \,\sigma_{12}\,\sigma_7+a\,{k_1 }^4 \,n\,\sigma_{12}\,\sigma_7+2\,a\,k_2 \,n^4 \,\sigma_{12}\,\sigma_7+a\,{k_2 }^4 \,n\,\sigma_{12}\,\sigma_7}{\sigma_{17}}+\frac{+a\,{k_1 }^2 \,n^3 \,\sigma_6\,\sigma_{12}-2\,a\,{k_1 }^3 \,n^2 \,\sigma_6\,\sigma_{12}+a\,{k_2 }^2 \,n^3 \,\sigma_6\,\sigma_{12}-2\,a\,{k_2 }^3 \,n^2 \,\sigma_6\,\sigma_{12}}{\sigma_{17}}+\frac{-4\,{k_1 }^2 \,{k_2 }^2 \,n\,\sigma_{12}\,\sigma_1 -4\,{k_1 }^2 \,{k_2 }^2 \,n^2 \,{\dot{x} }_0 \,\sigma_{11}+2\,a\,{k_1 }^2 \,n^3 \,\sigma_{11}\,\sigma_9+a\,{k_1 }^3 \,n^2 \,\sigma_{11}\,\sigma_9}{\sigma_{17}}+\frac{+2\,a\,{k_2 }^2 \,n^3 \,\sigma_{11}\,\sigma_9-a\,{k_2 }^3 \,n^2 \,\sigma_{11}\,\sigma_9+2\,a\,k_1 \,k_2 \,n^3 \,\sigma_{12}\,\sigma_7+2\,a\,k_1 \,{k_2 }^2 \,n^2 \,\sigma_6\,\sigma_{12}}{\sigma_{17}}+\frac{+2\,a\,{k_1 }^2 \,k_2 \,n^2 \,\sigma_6\,\sigma_{12}+2\,a\,{k_1 }^2 \,{k_2 }^2 \,n\,\sigma_6\,\sigma_{12}-a\,k_1 \,{k_2 }^2 \,n^2 \,\sigma_{11}\,\sigma_9+a\,{k_1 }^2 \,k_2 \,n^2 \,\sigma_{11}\,\sigma_9}{\sigma_{17}}+\frac{-2\,a\,k_1 \,{k_2 }^2 \,n^2 \,\sigma_{12}\,\sigma_7+2\,a\,{k_1 }^2 \,k_2 \,n^2 \,\sigma_{12}\,\sigma_7-2\,a\,{k_1 }^2 \,{k_2 }^2 \,n\,\sigma_{12}\,\sigma_7+4\,a\,k_1 \,k_2 \,n^3 \,\sigma_8\,\sigma_{11}}{\sigma_{17}}+\frac{+2\,a\,k_1 \,k_2 \,n^3 \,\sigma_6\,\sigma_{12}+4\,a\,k_1 \,k_2 \,n^3 \,\sigma_{11}\,\sigma_9+a\,k_1 \,{k_2 }^2 \,n^2 \,\sigma_8\,\sigma_{11}+a\,{k_1 }^2 \,k_2 \,n^2 \,\sigma_8\,\sigma_{11}}{\sigma_{17}}\\
\end{dmath}
%------------------------------------------------------------------------------------------------------------------------------------------------
\begin{dmath}
y(t) = \frac{3\,n^5 \,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }+\frac{3\,{k_1 }^4 \,n\,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }+\frac{3\,{k_2 }^4 \,n\,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }+\frac{a\,{k_1 }^3 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_1 }^3 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }-\frac{a\,{k_2 }^3 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }+\frac{3\,a\,{k_2 }^3 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }+\frac{a\,n^3 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }+\frac{3\,a\,n^3 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }-\frac{6\,{k_1 }^2 \,n^3 \,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }-\frac{6\,{k_2 }^2 \,n^3 \,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }+\frac{4\,{k_1 }^4 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }+\frac{4\,{k_2 }^4 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }+\frac{4\,n^4 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }-\frac{2\,{k_1 }^4 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }-\frac{2\,{k_2 }^4 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }-\frac{2\,n^4 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }-\frac{a\,{k_1 }^3 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_1 }^3 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }-\frac{a\,{k_2 }^3 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_2 }^3 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }-\frac{a\,n^3 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{3\,a\,n^3 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }+\frac{a\,k_1 \,{k_2 }^2 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{a\,{k_1 }^2 \,k_2 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{3\,a\,k_1 \,{k_2 }^2 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }+\frac{3\,a\,{k_1 }^2 \,k_2 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }+\frac{a\,k_1 \,n^2 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{a\,{k_1 }^2 \,n\,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{3\,a\,k_1 \,n^2 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }+\frac{a\,k_2 \,n^2 \,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_1 }^2 \,n\,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }+\frac{a\,{k_2 }^2 \,n\,x_0 \,\epsilon_12 }{2\,\epsilon_{15} }+\frac{3\,a\,k_2 \,n^2 \,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_2 }^2 \,n\,x_0 \,\epsilon_9 }{2\,\epsilon_{15} }-\frac{a\,{k_1 }^4 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{16} }-\frac{a\,{k_2 }^4 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{16} }-\frac{8\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }+\frac{3\,a\,n^4 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{16} }-\frac{8\,{k_1 }^2 \,n^2 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }-\frac{8\,{k_2 }^2 \,n^2 \,x_0 \,{\dot{y} }_0 \,\epsilon_{13}}{\epsilon_{15} }+\frac{4\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }+\frac{4\,{k_1 }^2 \,n^2 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }+\frac{4\,{k_2 }^2 \,n^2 \,x_0 \,{\dot{x} }_0 \,\epsilon_{14}}{\epsilon_{15} }-\frac{a\,k_1 \,{k_2 }^2 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }+\frac{3\,a\,k_1 \,{k_2 }^2 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }+\frac{a\,{k_1 }^2 \,k_2 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_1 }^2 \,k_2 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }-\frac{a\,k_1 \,n^2 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }+\frac{3\,a\,k_1 \,n^2 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }-\frac{a\,{k_1 }^2 \,n\,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_1 }^2 \,n\,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }+\frac{a\,k_2 \,n^2 \,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }-\frac{3\,a\,k_2 \,n^2 \,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }-\frac{a\,{k_2 }^2 \,n\,x_0 \,\epsilon_11 }{2\,\epsilon_{15} }-\frac{3\,a\,{k_2 }^2 \,n\,x_0 \,\epsilon_10 }{2\,\epsilon_{15} }+\frac{a\,{k_1 }^4 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{16} }+\frac{a\,{k_2 }^4 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{16} }-\frac{3\,a\,n^4 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{16} }-\frac{6\,{k_1 }^2 \,{k_2 }^2 \,n\,{x_0 }^2 \,\epsilon_{13}}{\epsilon_{15} }-\frac{a\,k_1 \,n^3 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_1 }^3 \,n\,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }-\frac{a\,k_2 \,n^3 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_2 }^3 \,n\,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,k_1 \,k_2 \,n\,x_0 \,\epsilon_12 }{\epsilon_{15} }+\frac{3\,a\,k_1 \,k_2 \,n\,x_0 \,\epsilon_9 }{\epsilon_{15} }-\frac{a\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }-\frac{a\,k_1 \,k_2 \,n\,x_0 \,\epsilon_11 }{\epsilon_{15} }-\frac{3\,a\,k_1 \,k_2 \,n\,x_0 \,\epsilon_10 }{\epsilon_{15} }+\frac{a\,k_1 \,n^3 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,{k_1 }^3 \,n\,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,k_2 \,n^3 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }+\frac{a\,{k_2 }^3 \,n\,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{4\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }+\frac{a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_4 }{{\left(k_1 -k_2 \right)}\,\epsilon_{15} }-\frac{4\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }-\frac{a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }-\frac{a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_3 }{{\left(k_1 +k_2 \right)}\,\epsilon_{15} }\\
\end{dmath}
%------------------------------------------------------------------------------------------------------------------------------------------------
\begin{equation}
    \dot{y}(t) = \frac{N_4}{D_4}
\end{equation}
where, \hfill
\begin{dmath}
N_4 = -6\,n^6 \,{x_0 }^2 \,\epsilon_{14} 
    - a\,{k_1 }^4 \,x_0 \,\epsilon_1 
    - a\,{k_2 }^4 \,x_0 \,\epsilon_1 
    + 3\,a\,n^4 \,x_0 \,\epsilon_1 
    + a\,n^4 \,x_0 \,\epsilon_7 
    + 3\,a\,n^4 \,x_0 \,\epsilon_6 
    + a\,{k_1 }^4 \,x_0 \,\epsilon_2 
    + a\,{k_2 }^4 \,x_0 \,\epsilon_2 
    - 3\,a\,n^4 \,x_0 \,\epsilon_2 
    + 12\,{k_1 }^2 \,n^4 \,{x_0 }^2 \,\epsilon_{14}
    - 6\,{k_1 }^4 \,n^2 \,{x_0 }^2 \,\epsilon_{14}
    + 12\,{k_2 }^2 \,n^4 \,{x_0 }^2 \,\epsilon_{14}
    - 6\,{k_2 }^4 \,n^2 \,{x_0 }^2 \,\epsilon_{14}
    - 4\,n^5 \,x_0 \,{\dot{x} }_0 \,\epsilon_{13}+a\,n^4 \,x_0 \,\epsilon_8 
    - 3\,a\,n^4 \,x_0 \,\epsilon_5 
    - 8\,n^5 \,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    - 4\,{k_1 }^4 \,n\,x_0 \,{\dot{x} }_0 \,\epsilon_{13}
    - 4\,{k_2 }^4 \,n\,x_0 \,{\dot{x} }_0 \,\epsilon_{13}
    - 2\,a\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,\epsilon_2 
    + 2\,a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_2 
    + 2\,a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_2 
    + a\,k_1 \,n^3 \,x_0 \,\epsilon_8 
    - a\,{k_1 }^3 \,n\,x_0 \,\epsilon_8 
    - 3\,a\,k_1 \,n^3 \,x_0 \,\epsilon_5 
    + a\,k_2 \,n^3 \,x_0 \,\epsilon_8 
    + 3\,a\,{k_1 }^3 \,n\,x_0 \,\epsilon_5 
    - a\,{k_2 }^3 \,n\,x_0 \,\epsilon_8 
    - 3\,a\,k_2 \,n^3 \,x_0 \,\epsilon_5 
    + 3\,a\,{k_2 }^3 \,n\,x_0 \,\epsilon_5 
    - 8\,{k_1 }^4 \,n\,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    - 8\,{k_2 }^4 \,n\,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    + 12\,{k_1 }^2 \,{k_2 }^2 \,n^2 \,{x_0 }^2 \,\epsilon_{14}
    + 2\,a\,k_1 \,n^3 \,x_0 \,\epsilon_1 
    - 2\,a\,{k_1 }^3 \,n\,x_0 \,\epsilon_1 
    + 2\,a\,k_2 \,n^3 \,x_0 \,\epsilon_1 
    - 2\,a\,{k_2 }^3 \,n\,x_0 \,\epsilon_1 
    + 8\,{k_1 }^2 \,n^3 \,x_0 \,{\dot{x} }_0 \,\epsilon_{13}
    + 8\,{k_2 }^2 \,n^3 \,x_0 \,{\dot{x} }_0 \,\epsilon_{13}
    - a\,k_1 \,n^3 \,x_0 \,\epsilon_7 
    + 3\,a\,k_1 \,n^3 \,x_0 \,\epsilon_6 
    + a\,{k_1 }^3 \,n\,x_0 \,\epsilon_7 
    - 3\,a\,{k_1 }^3 \,n\,x_0 \,\epsilon_6 
    + a\,k_2 \,n^3 \,x_0 \,\epsilon_7 
    - 3\,a\,k_2 \,n^3 \,x_0 \,\epsilon_6 
    - a\,{k_2 }^3 \,n\,x_0 \,\epsilon_7 
    + 3\,a\,{k_2 }^3 \,n\,x_0 \,\epsilon_6 
    + a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_8 
    + 3\,a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_5 
    + a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_8 
    + 3\,a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_5 
    + 16\,{k_1 }^2 \,n^3 \,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    + 16\,{k_2 }^2 \,n^3 \,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    + 2\,a\,{k_1 }^2 \,{k_2 }^2 \,x_0 \,\epsilon_1 
    - 2\,a\,k_1 \,n^3 \,x_0 \,\epsilon_2 
    + 2\,a\,{k_1 }^3 \,n\,x_0 \,\epsilon_2 
    + 2\,a\,k_2 \,n^3 \,x_0 \,\epsilon_2 
    - 2\,a\,{k_2 }^3 \,n\,x_0 \,\epsilon_2 
    - 2\,a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_1 
    - 2\,a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_1 
    - a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_7 
    - 3\,a\,{k_1 }^2 \,n^2 \,x_0 \,\epsilon_6 
    - a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_7 
    - 3\,a\,{k_2 }^2 \,n^2 \,x_0 \,\epsilon_6 
    - 2\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_7 
    - 6\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_6 
    - a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_7 
    + 3\,a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_6 
    + a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_7 
    - 3\,a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_6 
    - 16\,{k_1 }^2 \,{k_2 }^2 \,n\,x_0 \,{\dot{y} }_0 \,\epsilon_{14}
    + 8\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_2 
    - 2\,a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_2 
    + 2\,a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_2 
    - 2\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_8 
    + a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_8 
    + a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_8 
    - 6\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_5 
    - 3\,a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_5 
    - 3\,a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_5 
    + 8\,a\,k_1 \,k_2 \,n^2 \,x_0 \,\epsilon_1 
    + 2\,a\,k_1 \,{k_2 }^2 \,n\,x_0 \,\epsilon_1 
    + 2\,a\,{k_1 }^2 \,k_2 \,n\,x_0 \,\epsilon_1 
    + 8\,{k_1 }^2 \,{k_2 }^2 \,n\,x_0 \,{\dot{x} }_0 \,\epsilon_{13}
\end{dmath}
\begin{dmath}
    D_4 = {2\,{\left({k_1 }^4 -2\,{k_1 }^2 \,{k_2 }^2 -2\,{k_1 }^2 \,n^2 +{k_2 }^4 -2\,{k_2 }^2 \,n^2 +n^4 \right)}}
\end{dmath}
%------------------------------------------------------------------------------------------------------------------------------------------------

where, \hfill
% where, \hfill
\begin{center}
    \begin{math}
\begin{array}{cc}
     \sigma_1 =3\,x_0 \,n^2 +2\,{\dot{y} }_0 \,n+a\,\mathrm{cos}\left(\alpha_0 \right)\,\mathrm{sin}\left(\beta_0 \right) & 
     \sigma_2 =\mathrm{sin}\left(t\,{\left(k_1 -k_2 \right)}\right) \\
     \sigma_3 =\mathrm{sin}\left(t\,{\left(k_1 +k_2 \right)}\right) &
     \sigma_4 =\mathrm{cos}\left(t\,{\left(k_1 -k_2 \right)}\right) \\
     \sigma_5 =\mathrm{cos}\left(t\,{\left(k_1 +k_2 \right)}\right) &
     \sigma_6 =\mathrm{sin}\left(\alpha_0 +\beta_0 \right) \\
     \sigma_7 =\mathrm{sin}\left(\alpha_0 -\beta_0 \right) &
     \sigma_8 =\mathrm{cos}\left(\alpha_0 +\beta_0 \right) \\
     \sigma_9 =\mathrm{cos}\left(\alpha_0 -\beta_0 \right) &
     \sigma_{10} = 2\,n^2 \,{\left(k_1 +k_2 \right)}\,{\left(k_1 -k_2 \right)} \\
     \sigma_{11} = \mathrm{cos}\left(n\,t\right) &
     \sigma_{12} = \mathrm{sin}\left(n\,t\right) \\
     \multicolumn{2}{c}{\sigma_{13} = 2\,n^2 \,{\left(k_1 +k_2 -n\right)}\,{\left(k_1 -k_2 +n\right)}\,{\left(k_2 -k_1 +n\right)}\,{\left(k_1 +k_2 +n\right)}} \\
     \sigma_{14} = {2\,\left(k_1 -\,k_2 \right)}\,{\left(k_1 -k_2 +n\right)}\,{\left(k_2 -k_1 +n\right)} &
     \sigma_{15} = {2\,\left(\,k_1 +\,k_2 \right)}\,{\left(k_1 +k_2 -n\right)}\,{\left(k_1 +k_2 +n\right)} \\
\end{array}
\end{math}
\end{center}
%------------------------------------------------------------------------------------------------------------------------------------------------

\begin{center}
    \begin{math}
\begin{array}{cc}
     \epsilon_1 =\cos \left(-k_1 \,t-k_2 \,t+\alpha_0 +\beta_0 \right) & 
     \epsilon_2 =\cos \left(-k_1 \,t+k_2 \,t+\alpha_0 -\beta_0 \right)\\
     \epsilon_3 =\sin \left(-k_1 \,t-k_2 \,t+\alpha_0 +\beta_0 \right) &
     \epsilon_4 =\sin \left(-k_1 \,t+k_2 \,t+\alpha_0 -\beta_0 \right)\\
     \epsilon_5 =\cos \left(-n\,t+\alpha_0 +\beta_0 \right) &
     \epsilon_6 =\cos \left(n\,t-\alpha_0 +\beta_0 \right) \\
     \epsilon_7 =\cos \left(n\,t+\alpha_0 -\beta_0 \right) &
     \epsilon_8 =\cos \left(n\,t+\alpha_0 +\beta_0 \right) \\
     \epsilon_9 =\sin \left(-n\,t+\alpha_0 +\beta_0 \right)&
     \epsilon_{10} =\sin \left(n\,t-\alpha_0 +\beta_0 \right)\ \\
     \epsilon_{11} =\sin \left(n\,t+\alpha_0 -\beta_0 \right) &
     \epsilon_{12} =\sin \left(n\,t+\alpha_0 +\beta_0 \right) \\
     \epsilon_{13} =\cos \left(n\,t\right) & 
     \epsilon_{14} =\sin \left(n\,t\right) \\
     \multicolumn{2}{c}{\epsilon_{15} ={k_1 }^4 -2\,{k_1 }^2 \,{k_2 }^2 -2\,{k_1 }^2 \,n^2 +{k_2 }^4 -2\,{k_2 }^2 \,n^2 +n^4} \\
     \multicolumn{2}{c}{\epsilon_{16} =2\,{k_1 }^4 -4\,{k_1 }^2 \,{k_2 }^2 -4\,{k_1 }^2 \,n^2 +2\,{k_2 }^4 -4\,{k_2 }^2 \,n^2 +2\,n^4}
    %  \multicolumn{2}{c}{\sigma_{13} = 2\,n^2 \,{\left(k_1 +k_2 -n\right)}\,{\left(k_1 -k_2 +n\right)}\,{\left(k_2 -k_1 +n\right)}\,{\left(k_1 +k_2 +n\right)}} \\
\end{array}
\end{math}
\end{center}

%------------------------------------------------------------------------------------------------------------------------------------------------
\bibliographystyle{AAS_publication}   % Number the references.
\bibliography{references}   % Use references.bib to resolve the labels.

\end{document}
